Formalizing, Verifying and Applying ISA Security Guarantees as Universal Contracts

Progress has recently been made on specifying instruction set architectures (ISAs) in executable formalisms rather than through prose. However, to date, those formal specifications are limited to the functional aspects of the ISA and do not cover its security guarantees. We present a novel, general method for formally specifying an ISAs security guarantees to (1) balance the needs of ISA implementations (hardware) and clients (software), (2) can be semi-automatically verified to hold for the ISA operational semantics, producing a high-assurance mechanically-verifiable proof, and (3) support informal and formal reasoning about security-critical software in the presence of adversarial code. Our method leverages universal contracts: software contracts that express bounds on the authority of arbitrary untrusted code. Universal contracts can be kept agnostic of software abstractions, and strike the right balance between requiring sufficient detail for reasoning about software and preserving implementation freedom of ISA designers and CPU implementers. We semi-automatically verify universal contracts against Sail implementations of ISA semantics using our Katamaran tool; a semi-automatic separation logic verifier for Sail which produces machine-checked proofs for successfully verified contracts. We demonstrate the generality of our method by applying it to two ISAs that offer very different security primitives: (1) MinimalCaps: a custom-built capability machine ISA and (2) a (somewhat simplified) version of RISC-V with PMP. We verify a femtokernel using the security guarantee we have formalized for RISC-V with PMP.

==> src/revision.tex <==
\section{Revision}

Required changes for the revision:
\begin{itemize}
\item Properly situate the contributions in the context of the missing related work, which the authors already agreed should be included.
\item Better explain the novelty of this work, incorporating the arguments made in the author response front-and-centre in the paper.
\item Help the reader that is unfamiliar with memory capability and/or their safety and/or separation logic to follow the paper more easily. Even consider using, within reason appendices to support this or some glossary not of terms but of concepts. To gain space you may consider simplifying the case-studies on KATAMARAN using capabilities machines to 1 single case study.
\item Other improvements mentioned in the rebuttal
\end{itemize}

\subsection{Related Work}

We added the discussion regarding the missed related work in \secref{sec:intro} to better situate the novelty of our work.
\secref{sec:related-work} is also updated to include the missed related work.
We properly situate our RISC-V case study not as the first demonstration of UCs outside of the capability machine setting, but as demonstrating the generality of our method.

\subsection{Novelty}

We updated \secref{sec:universal-contracts} to emphasize the novelty of our method and focus on it being more general than shown in the related work.
Furthermore, we revised our contributions in light of the related work pointed out by the reviewers and rephrased it as reconciling two requirements with our approach: logic expressiveness and verification automation for authoritative, engineer-friendly interpreter-style ISA definitions.

\subsection{Background}

We moved, and expanded upon, our explanation of separation logic into its own background section.
We added a more intuitive description of a memory capability in terms of traditional pointers.
We made the discussion of Katamaran verification more accessible by avoiding some PL jargon and
better explaining and motivating the design.

\subsection{Capability safety}

We give a more intuitive explanation of capability safety in \secref{sec:capability-safety}.



==> src/riscv-pmp-security.tex <==
\section{Memory Integrity for RISC-V PMP}
\label{sec:risc-v-pmp}
In addition to \MinimalCaps{}, which is an artificial ISA defined by us, we demonstrate the generality of universal contracts and Katamaran by applying them to RISC-V with support for exceptions (synchronous interrupts) and the PMP extension, as explained in \secref{sec:background}.
The universal contract will capture the memory integrity guarantee offered by the ISA when invoking untrusted code. 

Our model of RISC-V is translated to \muSail{} from the ISA's canonical \Sail{} semantics with a
number of simplifications and assumptions:
% we assume unbounded integers,
only two (rather than 16 or
64) PMP configuration entries in top-of-range (TOR) mode are supported, there is no virtual memory, and we only support M-mode and U-mode.
%A WIP version of the model with bounded integers is included in the supplementary material.
%It includes working versions of the Katamaran-automated proofs, but does not yet have a working Iris model.

\begin{figure}[t]
  \begin{math}
  \begin{array}{l}
    \left\{
      \begin{array}{l}
        \mathit{Normal}(l,h,\mathit{mpp},\mathit{entries}) \\
        \astm \later (\mathit{CSR\ Modified}(l,\mathit{entries}) \wand \wpre{\mathit{fdeCycle()}}{~\mathit{True}~}) \\
        \astm \later (\mathit{Trap}(l,h,\mathit{entries}) \wand \wpre{\mathit{fdeCycle()}}{~\mathit{True}~}) \\
        \astm \later (\mathit{Recover}(l,h,\mathit{mpp},\mathit{entries}) \wand \wpre{\mathit{fdeCycle()}}{~\mathit{True}~})
        %% Explicit form
%%         \exists c, \mathit{mcause}         \mapsto c
%%         \astm      \mathit{cur\_privilege} \mapsto p
%%         \astm      \mathit{nextpc}         \mapsto \mathit{npc} \\
%%         \astm      \mathit{pc}             \mapsto i
%%         \astm      \mathit{mtvec}          \mapsto h
%%         \astm      \mathit{mstatus}        \mapsto [ mpp ] \\
%%         \astm      \mathit{mepc}           \mapsto \mathit{mepc}
%%         \astm      \mathit{PMP\_entries\ entries} \\
%%         \astm      \mathit{PMP\_addr\_access\ entries\ p}
%%         \astm      \mathit{GPRS} \\
%% %%         \astm \later ((        \mathit{mcause}         \mapsto 
%%          \astm          \mathit{cur\_privilege} \mapsto p \\
%%          \astm\ (\exists \mathit{npc}, \mathit{nextpc} \mapsto \mathit{npc}
%%          \astm      \mathit{pc}             \mapsto \mathit{npc})
%%          \astm      \mathit{mtvec}          \mapsto h \\
%%          \astm      \mathit{mstatus}        \mapsto [ mpp ]
%%          \astm      \mathit{mepc}           \mapsto \mathit{mepc} \\
%%          \astm      \mathit{PMP\_entries\ entries}
%%          \astm      \mathit{PMP\_addr\_access\ entries\ p} \\
%%          \astm      \mathit{GPRS}) \wand \mathit{wp\ fdeCycle()\ ~\mathit{True}~})
%%         \astm \ldot
      \end{array}
    \right\} \\
    \mathit{fdeCycle()} \left\{
        ~\mathit{True}~
    \right\}
  \end{array}
  \end{math}%
  \begin{multline*}
    \mathit{Normal}(m,h,\mathit{mpp},\mathit{entries}) =\\
                                                \left\{
                                                \begin{alignedat}{1}
                                                  &(\exists i\ldotp \mathit{pc}             \mapsto i) \astm
                                                    \mathit{cur\_privilege} \mapsto l \astm
                                                    \mathit{mtvec}          \mapsto h \astm\\
                                                  &(\exists c\ldotp \mathit{mcause}         \mapsto c) \astm
                                                    \mathit{mstatus}        \mapsto [ mpp ] \astm \\
                                                  &\mathit{mepc}           \mapsto \mathit{mepc} \astm
                                                    \mathit{PMP\_entries\ entries} \astm \\
                                                  &\Sep_{r \in \mathrm{GPR}}\left(\exists w\ldotp r \mapsto w \right) \astm
                                                    \mathit{PMP\_addr\_access\ entries\ l}
                                                \end{alignedat} \right.
  \end{multline*}%
  \begin{multline*}
    \mathit{Trap}(l,h,\mathit{entries}) =\\
                                                \left\{
                                                \begin{alignedat}{1}
                                                  &\mathit{pc}             \mapsto h \astm
                                                    \mathit{cur\_privilege} \mapsto \mathit{Machine} \astm
                                                    \mathit{mtvec}          \mapsto h \astm\\
                                                  &(\exists c\ldotp \mathit{mcause}         \mapsto c) \astm
                                                    \mathit{mstatus}        \mapsto [ l ] \astm \\
                                                  &(\exists c\ldotp \mathit{mepc}           \mapsto c) \astm
                                                    \mathit{PMP\_entries\ entries} \astm \\
                                                  &\Sep_{r \in \mathrm{GPR}}\left(\exists w\ldotp r \mapsto w \right) \astm
                                                    \mathit{PMP\_addr\_access\ entries\ l}
                                                \end{alignedat}
                                                                            \right.
  \end{multline*}

  \caption{Universal Contract for Memory Integrity for RISC-V with PMP}
  \label{fig:riscvcontract}
\end{figure}

We define the universal contract for this machine, over the fetch-decode-execute cycle as shown in \figref{fig:riscvcontract}.
In this contract the machine starts from a Normal state, which requires ownership (and knowledge of the current values) of the architectural registers $\mathit{pc}$, $\mathit{cur\_privilege}$, $\mathit{mtvec}$, $\mathit{mcause}$, $\mathit{mstatus}$ and $\mathit{mepc}$, containing respectively the program counter, current privilege level, configured exception handler address, cause of the last interrupt, and the privilege level and program counter before the last interrupt.
Additionally, the state requires ownership of the general-purpose registers and the current PMP configuration entries.
Finally and perhaps most importantly, \textbf{Normal} requires ownership of PMP\_addr\_access entries p, an abstract predicate that represents ownership of the part of memory that is accessible according to the PMP policy entries (discussed further below).

Given this authority, the contract states that the ISA will execute correctly, provided that three extra conditions are fulfilled.
All three require that the machine continues executing correctly in a specific situation: (1) when CSRs are modified, (2) when a trap occurs to the exception handler, and (3) when an MRET is used to return to a lower privilege level (Recover).
The three conditions use the standard \Iris{} predicate $\wpre{\mathit{fdeCycle()}}{~\mathit{True}~}$ which represents the \emph{weakest precondition} for $\mathit{fdeCycle()}$ to execute correctly without breaking any invariants.
\steve{The magic wand was already used in the previous section, so maybe this should be moved.}
They also use the separating implication operator $\wand$ (affectionately referred to as the \emph{magic wand}) to require that this weakest precondition holds when authority for the respective premises is presented.

For brevity, we only show the definition of Trap, arguably the most important case, as the other two cases can only be reached if the original privilege level l was Machine, \ie{} the UC is used to reason about untrusted Machine code.
PMP can encapsulate Machine code (by locking PMP entries) but more typically encapsulates lower-privilege code.
Trap requires ownership of the same ISA registers and memory as Normal above.
However, it additionally requires that the program counter is set to the configured exception handler, that cur\_privilege is set to Machine mode, and that mstatus correctly stores l as the previous privilege level.
Under these conditions, the user of the UC needs to prove that the machine will execute correctly.
This reflects the intuition that trusted code can rely on PMP to encapsulate untrusted lower-privilege code, but only if it ensures security of the configured exception handler.

\begin{figure}[b]
  \begin{math}
    \begin{array}{l}
      \mathit{PMP\_addr\_access\ entries\ m} = \\
      \quad \Sep_{a \in addrs}
      ((\exists p, PMP\_access\ a\ entries\ m\ p) \wand \exists w, a \mapsto w)
    \end{array}
  \end{math}

  \caption{PMP\_addr\_access predicate implementation}
  \label{fig:pmpaddraccess}
\end{figure}

A crucial predicate in the universal contract is $\mathit{PMP\_addr\_access}$, which captures the semantics of the PMP check algorithm and is shown in \figref{fig:pmpaddraccess}.
It is defined as a separating conjunction over all addresses of the machine.
The predicate allows obtaining a pointsto predicate for an address $a$, if the PMP policy specifies a permission $p$ (e.g.\ \emph{Read} or \emph{Write})for it at privilege level l.
Importantly, this means that ownership of other memory locations is not required for using the universal contract.

\subsection{Verification}
\label{sec:riscv-verification}

\begin{figure}%[b]
  \footnotesize
  \begin{alignat*}{2}
    \left\{
    \begin{array}{l}
      \mathit{Read} \sqsubseteq t \\
      \astm \mathit{cur\_privilege} \mapsto p \\
      \astm \mathit{PMP\_entries\ entries} \\
      \astm \mathit{PMP\_access\ a\ entries\ p\ t} \\
      \astm a \mapsto w
    \end{array}
    \right\}
    &\,\mathit{read\_ram\ a}\,&
    \left\{\begin{array}{l}
      \mathit{cur\_privilege} \mapsto p \\
      \astm \mathit{PMP\_entries\ entries} \\
      \astm a \mapsto w
    \end{array} \right\} \\
    \left\{
    \begin{array}{l}
      \mathit{Write} \sqsubseteq t \\
      \astm \mathit{cur\_privilege} \mapsto p \\
      \astm \mathit{PMP\_entries\ entries} \\
      \astm \mathit{PMP\_access\ a\ entries\ p\ t} \\
      \astm \exists w, a \mapsto w
    \end{array}
    \right\}
    &\,\mathit{write\_ram\ a\ v}\,&
    \left\{\begin{array}{l}
      \mathit{cur\_privilege} \mapsto p \\
      \astm \mathit{PMP\_entries\ entries} \\
      \astm a \mapsto v
    \end{array} \right\}
  \end{alignat*}
\caption{Contracts for functions interacting directly with memory}
\label{fig:ramcontracts}
\end{figure}

As for \MinimalCaps{}, we verify that our universal contract holds for the functional specification of RISC-V.
This verification is done assuming contracts for reading from and writing to memory, shown in \figref{fig:ramcontracts}.
The contracts require read or write access, respectively in the form of the $\mathit{PMP\_access}$ predicate encountered above.
We also require that we have ownership of the address that we want to read from or write to, $a \mapsto w$.
The postconditions of these functions return the resources used, updated in the case of $\mathit{write\_ram}$ to point to the newly written value.

\begin{figure*}[t]
  \centerline{\includegraphics[width=2.2\columnwidth]{images/risc-v-state-machine.png}}
  \caption{Contract for taking a step on RISC-V (\ie executing an instruction). New existentially quantified logic variables are shown in red, modified registers are shown in bold.
    Constraints on the Start of Iteration logic variables are indicated on the arrows (we require for CSR Modified and Recover state transitions that we started from a state running
    in Machine mode, \ie $p = \mathit{Machine}$).}
  \label{fig:instrexeccontract}
\end{figure*}

Like for \MinimalCaps{}, the proof of the universal contract works by iterating a contract for the single-cycle {fdeStep()} function.
The contract is depicted in a bit more detail in \figref{fig:instrexeccontract}.
It specifies that executing an instruction will leave the CPU in one of the states Normal, CSRModified, Trap or Recover which we already encountered in the UC, with specific values for the ISA registers.
Not shown are the predicates for ownership over the general-purpose registers, \ie $\Sep_{r \in \mathrm{GPR}}\left(\exists w\ldotp r \mapsto w \right)$, and the PMP entries, $\mathit{PMP\_entries}$, and $\mathit{PMP\_addr\_access}$, representing ownership of the PMP-authorized memory.
All these predicates are preserved as-is upon a state change, except $\mathit{PMP\_entries}$ which may be modified in the \textbf{CSR Modified} state.
The CSRModified and Recover states can only be reached when executing in \emph{Machine} mode, \ie $p = \mathit{Machine}$.
Trap transfers into \emph{Machine} mode and Recover returns to the privilege level stored in mpp.

\begin{figure*}[t]
  \footnotesize
  \begin{math}
    \begin{array}{r l l}
    \braced{\mathit{PMP\_entries\ entries}}
    &\,\mathit{open\_PMP\_entries}\,&
    \left\{
    \begin{array}{l}
      \exists \mathit{cfg_0,\ addr_0,\ cfg_1,\ addr_1,\ } \\
      (\mathit{pmp_0cfg} \mapsto \mathit{cfg_0} \astm
      \,\mathit{pmpaddr_0} \mapsto \mathit{addr_0} \astm \\
      \,\mathit{pmp_1cfg} \mapsto \mathit{cfg_1} \astm
      \,\mathit{pmpaddr_1} \mapsto \mathit{addr_1} \astm \\
      \,\mathit{entries} = [(\mathit{cfg_0}, \mathit{addr_0}); (\mathit{cfg_1}, \mathit{addr_1})])
    \end{array}
    \right\} \\[1em]
    \left\{
    \begin{array}{l}
      \mathit{PMP\_addr\_access\ entries\ p} \astm \\
      0 \leq \mathit{addr} \leq \mathit{maxAddr} \astm \mathit{PMP\_access\ addr\ entries\ p\ acc}
    \end{array}
    \right\}
    &\,\mathit{extract\_PMP\_ptsto}\,&
    \left\{
      \exists w\ldotp \mathit{addr} \mapsto w \astm (\mathit{addr} \mapsto w \wand \mathit{PMP\_addr\_access\ entries\ p})
    \right\} \\[1em]
    \left\{
      \exists w\ldotp \mathit{addr} \mapsto w \astm (\mathit{addr} \mapsto w \wand \mathit{PMP\_addr\_access\ entries\ p})
    \right\}
    &\,\mathit{return\_PMP\_ptsto}\,&
    \left\{
      \mathit{PMP\_addr\_access\ entries\ p}
    \right\}
  \end{array}
  \end{math}
  \caption{Contracts for lemmas used in RISC-V PMP case study.}
  \label{fig:riscvlemmas}
\end{figure*}

To verify the memory integrity property for RISC-V with PMP, we define some lemmas that aid in the semi-automatic verification of the case.
\figref{fig:riscvlemmas} depicts some interesting lemmas concerning the PMP extension.
The first lemma $\mathit{open\_PMP\_entries}$ and a dual lemma called $\mathit{close\_PMP\_entries}$, open resp.\ close the $\mathit{PMP\_entries}$ predicate, to allow direct access to the PMP CSRs in parts of the ISA semantics that access them, particularly the PMP check algorithm.
We use the same scheme for reasoning about GPRs, \ie we pack them in a predicate and open and close it when appropriate.
The two lemmas needed for interacting with memory are $\mathit{extract\_PMP\_ptsto}$ and $\mathit{return\_PMP\_ptsto}$.
$\mathit{extract\_PMP\_ptsto}$ trades ownership of PMP-authorized memory, given by $\mathit{PMP\_addr\_access}$ for a pointsto chunk for an authorized, in-range address $a$ and a magic wand that allows to recover $\mathit{PMP\_addr\_access}$ using $\mathit{return\_PMP\_ptsto}$ if we return the pointsto chunk.
All these lemmas are proven correct in the \Iris{} model of our case and are explicitly invoked in its function definitions using ghost statements that aid the semi-automatic verification of the contracts of these functions by \Katamaran{}.

These lemma invocations suffice to let Katamaran verify most of the contracts in the codebase.
As for MinimalCaps, we only need to prove the contract for fdeCycle() and its lemmas manually, because it requires the use of \Iris{}'s later modality and L\"ob induction, which Katamaran does not (yet) support.
\steve{I can't find the discussion of manual proofs of lemmas and fdeCycle in the MinimalCaps section.}
The contract expresses PMP's intuitive security guarantee and remains agnostic of software-defined abstractions.
Nevertheless, we will see in Section~\ref{sec:femtokernel} that it can be used to reason about specific security-critical code relying on PMP security guarantees.


==> src/universal-contracts.tex <==
\section{Universal Contracts for \Sail{} ISA semantics}
\label{sec:universal-contracts}
Although the general approach has not been previously described in the literature, universal contracts have been used before to formalize security guarantees for high-level languages \citep{van2019linear,devriese2016reasoning,swasey2017robust} as well as assembly languages \citep{skorstengaard2018reasoning,georges2021efficient,van_strydonck_proving_2022}.
Essentially, the idea is to formulate the security guarantees offered by a programming language or ISA in the form of a contract that holds for arbitrary, potentially untrusted, code, \ie{} a universal contract.
The contract expresses the restrictions enforced by the language on untrusted programs and needs to be proven to hold under the language's operational semantics.

Universal contracts are formalized using separation logic, an extension of Hoare logic that enables reasoning about programs that use shared mutable data structures, such as the heap \citep{reynolds2002separation}.
Furthermore, separation logic can be used for sequential and for concurrent programs.
The universal contract is a Hoare triple over an arbitrary piece of code, where the precondition and postcondition describe the conditions that need to be met and the guarantees given when executing the code.
%This allows the specification of universal contracts for which we can impose an initial configuration need to uphold a guarantee, before executing some code.\domi{this sentence doesn't parse?} \sand{I think it's just a first draft of the sentence I wrote above, it is saying the exact same thing} 
We will make this more concrete in the case studies discussed in \secref{sec:capability-safety} and \secref{sec:risc-v-pmp}.

%We present universal contracts as a Hoare triple over arbitrary code: $\hoare{\mathit{Security~Guarantee}}{\knowInv{}{\mathit{code}}}{\mathit{Security~Guarantee}}$.
%\domi{I don't like this representation (with ``security guarantee'' as pre- and postcondition), as the precondition and postcondition are not security guarantees in themselves, but it's the triple as a whole that constitutes the security guarantee (under some conditions, some things are guaranteed).}
While universal contracts apply to arbitrary assembly code, they take a slightly different form in our setting.
When using \Sail{}, an ISA semantics is defined through a definitional interpreter for the ISA's assembly language, with a main function that implements the fetch-decode-execute cycle of the ISA.
The arbitrary programs that our contract applies to therefore take the form of arbitrary instructions encoded in memory.
Our universal contract is thus defined as a Hoare triple over the \emph{Fetch-Decode-Execute cycle}.
In the remainder of this paper, we will use the function name \emph{fdeCycle} to refer to the \Sail{} function implementing this cycle, even though it may be named differently in a particular \Sail{} spec.%\domi{Does fdeCycle() execute one FDE cycle or does it keep running cycles indefinitely? Sander: it keeps running indefinitely}
%% This means that we end up with a universal contract for an ISA in the following form:
%% \begin{displaymath}
%%   \begin{array}{l}
%%     \braced{Security~Guarantee} \\
%%     \mathit{Fetch-Decode-Execute\ cycle} \\
%%     \braced{Security~Guarantee}
%%   \end{array}
%% \end{displaymath}

The goals of our approach are to enable reasoning about the ISA and programs written in it, as well as preserving freedom of implementation.
In other words, we want to define universal contracts for the security guarantees offered by an ISA but leave them sufficiently abstract so that they remain valid under ISA modifications.

Although we verify universal contracts against an ISA's operational semantics, that does not mean it should be considered as derivative or subjugate.
Rather, the UC should be regarded as a \emph{security specification}, supplementing the functional specification of the ISA.
This security specification is part of the ISA contract and precludes future and current ISA implementations and extensions from adding instructions or other behavior that violate the ISA guarantees, while otherwise preserving their implementation freedom.

We conjecture that the universal contracts defined in the case studies presented later in this paper are sufficiently abstract to allow a range of extensions.
For instance, in the case of RISC-V, for which we currently define a contract over the base instruction set and the PMP extension, the universal contract should hold for more optional features of the ISA and extensions (for example adding a floating point unit, user-level interrupts etc.) without requiring major changes to the universal contract.
Of course, not all modifications or extensions will be supported by the same universal contract.
New semantic features, for example virtual memory, will require modifying the universal contract accordingly.

Ideally, the effort to re-verify a universal contract for a modified ISA with a program verifier is kept minimal.
It is commonly understood that a high degree of proof automation leads to proofs that are \emph{robust} to changes \citep{cpdt,logicalfoundations}.
Therefore, for small modifications or modifications that are orthogonal to security-related matters, we should expect that a semi-automatic verifier, as we present in \secref{sec:katamaran}, can re-verify proofs with no or only a minimal amount of intervention.

% Having such a security specification supports verifying that the security specification holds against a modified version of the ISA.
% Unless semantic features of the ISA are changed or added, a semi-automatic verifier, as we present in \secref{sec:katamaran}, should be able to verify that the security guarantees still hold without modifications to the proofs.
% %\sand{not happy about the above, its a claim that we don't currently prove... (but I do explain it for the risc-v case study below, is that enough to make reader believe this to be true?}
% % \steve{Proof automation (in contrast to manual proofs) results in proofs that are \emph{robust} to changes. Robust meaning most likely to still work or with a minimal amount of intervention but not guaranteed to. We can cite Bedrock and so on. Did we have another citation somewhere?}
% \steve{I think these paragraphs jump between ideas. I think best would be to distinguish between the idea that a universal contracts that is abstract enough so that it still holds under some modifications/extensions and the actual (re-)verification of that universal contract in a verifier.}
% \steve{Integrate the following: Ideally, the effort to re-verify the modified ISA is kept minimal.
%   It is understood, that a high degree of proof automation, leads to proofs that are \emph{robust} to changes \citep{cpdt,logicalfoundations}.
%   Therefore, for small modifications or modifications that are orthogonal to security-related matters, we should expect that a semi-automatic verifier, as we present in \secref{sec:katamaran}, can re-verify proofs with no or only a minimal amount of intervention.
% }
% For the case studies we present later in this paper, this means that the universal contracts we've verified should still hold once additional instructions  have been added to the ISA cases.
% In the case of RISC-V, for which we currently define a contract over the base instruction set and the PMP extension, we can extend the case study to a larger ISA (for example adding a floating point unit, user-level interrupts etc.) without requiring changes to the universal contract.
% Not all modifications or extensions will be supported by the same universal contract.
% New semantic features, for example virtual memory, will require modifying the universal contract accordingly.

% \domi{I have trouble imagining what kind of properties or settings you have in mind in the following sentence, I propose to remove it. }
% We conclude this section with the remark that while our focus is on universal contracts for \Sail{} ISA semantics, they can be applied in other settings as well where one wants to reason about properties maintained when executing an arbitrary piece of code.

%% TODO: Feedback
%% Goals should be clear and well-explained
%% See notes domi on abstact, but push them through introduction, entire paper



